Effects of context, complexity, and clustering on evaluation for math formula retrieval

There are now several test collections for the formula retrieval task, in which a system's goal is to identify useful mathematical formulae to show in response to a query posed as a formula. These test collections differ in query format, query complexity, number of queries, content source, and relevance definition. Comparisons among six formula retrieval test collections illustrate that defining relevance based on query and/or document context can be consequential, that system results vary markedly with formula complexity, and that judging relevance after clustering formulas with identical symbol layouts (i.e., Symbol Layout Trees) can affect system preference ordering.

==> references.tex <==
@inproceedings{ntcir10,
  title={{NTCIR-10 Math Pilot Task Overview}},
  author={Aizawa, Akiko and Kohlhase, Michael and Ounis, Iadh},
  booktitle={Proceedings of the 10th NTCIR Conference},
    pages={654--661},
  year={2013}
}
@inproceedings{aizawa2014ntcir,
  title={{NTCIR-11 Math-2 Task Overview}},
  author={Aizawa, Akiko and Kohlhase, Michael and Ounis, Iadh and Schubotz, Moritz},
  booktitle={Proceedings of the 11th NTCIR Conference},
  pages={88--98},
  year={2014},
}

@inproceedings{avenoso2021xy,
  title={{XY-PHOC Symbol Location Embeddings for Math Formula Retrieval and Autocompletion}},
  author={Avenoso, Robin and Mansouri, Behrooz and Zanibbi, Richard},
    booktitle={Working Notes of CLEF 2021-Conference and Labs of the Evaluation Forum},
  year={2021}
}

@inproceedings{davila2017layout,
  title={{Layout and Semantics: Combining Representations for Mathematical Formula Search}},
  author={Davila, Kenny and Zanibbi, Richard},
  booktitle={Proceedings of the 40th International ACM SIGIR Conference on Research and Development in Information Retrieval},
    pages={1165--1168},
  year={2017},
}

@inproceedings{diaz2021mathdeck,
  title={{The MathDeck Formula Editor: Interactive Formula Entry Combining LaTeX, Structure Editing, and Search}},
  author={Diaz, Yancarlos and Nishizawa, Gavin and Mansouri, Behrooz and Davila, Kenny and Zanibbi, Richard},
  booktitle={Extended Abstracts of the 2021 CHI Conference on Human Factors in Computing Systems},
    pages={1--5},
  year={2021}
}

@inproceedings{mansouri2019tangent,
  title={{Tangent-{CFT}: An Embedding Model for Mathematical Formulas}},
  author={Mansouri, Behrooz and Rohatgi, Shaurya and Oard, Douglas W and Wu, Jian and Giles, C Lee and Zanibbi, Richard},
  booktitle={Proceedings of the 2019 ACM SIGIR International Conference on Theory of Information Retrieval},
  year={2019},
    pages={11--18},
  organization={ACM}
}

@inproceedings{mansouri2019characterizing,
  title={{Characterizing Searches for Mathematical Concepts}},
  author={Mansouri, Behrooz and Zanibbi, Richard and Oard, Douglas W},
  booktitle={2019 ACM/IEEE Joint Conference on Digital Libraries (JCDL)},
  year={2019},
  organization={IEEE}
}

@inproceedings{mansouri2020dprl,
  title={{DPRL Systems in the {CLEF} 2020 {ARQMath} Lab}},
  author={Mansouri, Behrooz and Oard, Douglas W and Zanibbi, Richard},
  booktitle={Working Notes of CLEF 2020-Conference and Labs of the Evaluation Forum},
  year={2020}
}

@inproceedings{mansouri2021ltr,
  title={{Learning to Rank for Mathematical Formula}},
  author={Mansouri, Behrooz and Zanibbi, Richard and Oard, Douglas W},
  booktitle={Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages = {952–961},
  year={2021}
}
@inproceedings{mansouri2021overview,
  title={{Overview of {ARQMath}-2 (2021): Second {CLEF} Lab on Answer Retrieval for Questions on Math}},
  author={Mansouri, Behrooz and Zanibbi, Richard and Oard, Douglas W and Agarwal, Anurag},
  booktitle={Experimental IR Meets Multilinguality, Multimodality, and Interaction: 12th International Conference of the CLEF Association},
  pages={215--238},
  year={2021},
  organization={Springer}
}
@inproceedings{ng2021dowsing,
  title={{Dowsing for Answers to Math Questions: Ongoing Viability of Traditional MathIR}},
  author={Ng, Yin Ki and Fraser, Dallas J and Kassaie, Besat and Tompa, Frank Wm},
    booktitle={Working Notes of CLEF 2021-Conference and Labs of the Evaluation Forum},
  year={2021}
}

@inproceedings{sakai2007alternatives,
  title={{Alternatives to Bpref}},
  author={Sakai, Tetsuya},
  booktitle={Proceedings of the 30th annual international ACM SIGIR Conference on Research and Development in Information Retrieval},
    pages={71--78},
  year={2007}
}

@inproceedings{zanibbi2016ntcir,
  title={{NTCIR-12 MathIR Task Overview}},
  author={Zanibbi, Richard and Aizawa, Akiko and Kohlhase, Michael and Ounis, Iadh and Goran Topic and Davila, Kenny},
  booktitle={Proceedings of the 12th NTCIR Conference},
    pages={299--308},
  year={2016}
}

@inproceedings{zanibbi2020overview,
  title={{Overview of {ARQMath} 2020: {CLEF} Lab on Answer Retrieval for Questions on Math}},
  author={Zanibbi, Richard and Oard, Douglas W and Agarwal, Anurag and Mansouri, Behrooz},
  booktitle={Experimental IR Meets Multilinguality, Multimodality, and Interaction
Proceedings of the 11th International Conference of the CLEF Association},
  year={2020},
   pages={169--193},
  organization={Springer}
}

@inproceedings{zhong2019structural,
  title={{Structural Similarity Search for Formulas Using Leaf-Root Paths in Operator Subtrees}},
  author={Zhong, Wei and Zanibbi, Richard},
  booktitle={European Conference on Information Retrieval},
    pages={116--129},
  year={2019},
}
